A Method for the Runtime Validation of AI-based Environment Perception in Automated Driving System

Environment perception is a fundamental part of the dynamic driving task executed by Autonomous Driving Systems (ADS). Artificial Intelligence (AI)-based approaches have prevailed over classical techniques for realizing the environment perception. Current safety-relevant standards for automotive systems, International Organization for Standardization (ISO) 26262 and ISO 21448, assume the existence of comprehensive requirements specifications. These specifications serve as the basis on which the functionality of an automotive system can be rigorously tested and checked for compliance with safety regulations. However, AI-based perception systems do not have complete requirements specification. Instead, large datasets are used to train AI-based perception systems. This paper presents a function monitor for the functional runtime monitoring of a two-folded AI-based environment perception for ADS, based respectively on camera and LiDAR sensors. To evaluate the applicability of the function monitor, we conduct a qualitative scenario-based evaluation in a controlled laboratory environment using a model car. The evaluation results then are discussed to provide insights into the monitor's performance and its suitability for real-world applications.

==> old-texts/backup-concept.tex <==
% --- Original version of the AI Perception Validator algorithm in pseudocode
\IncMargin{1em}
    %\begin{mutic}}
    \begin{algorithm}
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{UpdateObjectList}{UpdateObjectList}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \KwData{\\1) Object list  \emph{CAI} received from Camera based AI\ based\ perception.\\
              2) Object list \emph{LAI} received from LiDAR based AI\ based\ perception.\\ 
              3) \emph{Safe-Zone}, Which is the region of interest is received from Safe-Zone component.
              }

    \Input{list\ CAI, list\ LAI, \emph{SafeZone}}
    \Output{A boolean, \emph{True} or \emph{False}}
    \BlankLine
    $local-cai = [\ ]$\ ,
    $local-lai = [\ ]$ \\
    $Valid   = True$\ ;\ $Removed = False$\\
    $\textbf{Initialize: }the\ thrsholds\ limits for\ comparison\ are:$\\
    $timeout$,\ $timestamp$\_$limit$,\  $width$\_$limit$,\ $height$\_$limit$,\ $distance$\_$limit$ 
    \BlankLine
     \caption{$Initialization\ of\ all\ inputs$}\label{algo_function_monitor_1}
    \end{algorithm}
    %\columnbreak
%---------------------------------------------------------------------------------------------------


    \begin{algorithm}
    
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{UpdateObjectList}{UpdateObjectList}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    $timestamp = CAI.timestamp$\\
    
    \For{$obj_i\ in\ the\ list\ CAI$}{
    $object= OBJECT3D$ \\
        $Assign\ all\ the\ attributes\ from\ obj_i\ to\ object$\\
        $object.matched=False$\\
        $object.timestamp=timestamp$\\
        \If{$object\ in\ SafeZone$}{
        $push\ object\ to\ local-cai[\ ]$
        }
        
    }
    \caption{$Part1:\ AI\ perception\ Validator$}\label{algo_function_monitor_2}
    \end{algorithm}
    
    \DecMargin{1em}
    %\end{multicols}
%-------------------------------------------------------------------------------------------------------------

    \begin{algorithm}
    
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{UpdateObjectList}{UpdateObjectList}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    $timestamp = LAI.timestamp$\\
    
    \For{$obj_j\ in\ the\ list\ LAI$}{
    $object= OBJECT3D$ \\
        $Assign\ all\ the\ attributes\ from\ obj_j\ to\ object$\\
        $object.matched=False$\\
        $object.timestamp=timestamp$\\
        \If{$object\ in\ SafeZone$}{
        $push\ object\ to\ local-lai[\ ]$
        }
        
    }
    \caption{$Part2:\ AI\ perception\ Validator$}\label{algo_function_monitor_3}
    \end{algorithm}
    \DecMargin{1em}
    %---------------------------------------------------------------------------------------------------------%

    
    \begin{algorithm}
    
    \DontPrintSemicolon
    \SetKwFunction{FUpdate}{FilterObjectList}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FUpdate{$SafeZone$, $ObjectList$, $LocalList$}}{
        $timestamp = ObjectList.timestamp$\\
    
        \For{$obj_i\ in\ the\ list\ ObjectList$}{
        $object= OBJECT3D$ \\
            $Assign\ all\ the\ attributes\ from\ obj_i\ to\ object$\\
            $object.matched=False$\\
            $object.timestamp=timestamp$\\
            \If{$object\ in\ SafeZone$}{
            $push\ object\ to\ LocalList$
            }
            
        }
    
        \KwRet $LocalList$\;
        }
    \caption{$Filter\ Object\ list\ $}\label{algo_function_monitor_2}
    \end{algorithm}

    %----------------------------------------------------------------------------------
    \IncMargin{1em}
    %\begin{mutic}}
    %\columnbreak
  
    \begin{algorithm}
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwFunction{Union}{Union}\SetKwFunction{FilterObjectList}{FilterObjectList}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    
    $local-cai=FilterObjectList(SafeZone,CAI,local-cai)$\\
    $local-lai=FilterObjectList(SafeZone,LAI,local-lai)$
    $cTime = getCurrentTime()$
    
    \BlankLine
    \If{$local-lai$ $and$ $local-cai$ $are\ both\ empty$ }{\label{lt}
    \KwRet Valid\\     
    }
    
    \For{$i \leftarrow obj_0$ \KwTo $last$ $obj_n$ $in$ $local-lai$}{
    \If{$cTime\ -\  obj_i.timestamp\ >\ timeout$ }{
    \If{$obj_i.matched\ != True$}{ 
    $Valid=False$\\

    }
    $remove\ obj_i\ from\ local-lai$
    $removed= True$\\
    }
    \lElse{$iterate\ to\ the\ next\ object\ obj_{i+1}\ in\ local-lai$}
    
    }

    % new for loop
    %\columnbreak
    \BlankLine
    \For{$j \leftarrow obj_0$ \KwTo $last$ $obj_m$ $in$ $local-cai$}{
    \If{$cTime\ -\  obj_j.timestamp\ >\ timeout$ }{
    \If{$obj_j.matched\ != True$}{ 
    $Valid=False$\\
    }
    $remove\ obj_j\ from\ local-cai$
    $removed= True$\\
    }
    \lElse{$iterate\ to\ the\ next\ object\ obj_{j+1}\ in\ local-cai$}
    
    }
    % done with the two for loop ///
    \BlankLine
    \For{$i \leftarrow obj_0$ \KwTo $last$ $obj_n$ $in$ $local-lai$}{
    $obj_{lidar} = obj_i$\\
    \For{$j \leftarrow obj_0$ \KwTo $last$ $obj_m$ $in$ $local-cai$}{
    
    $obj_{camera} = obj_i$\\
    \If{$obj_{lidar}.class_id == obj_{camera}.class_id\ \\ and\ difference(\ obj_{lidar}.timestamp,
    obj_{camera}\.timestamp) < timestamp$\_$limit\\ 
    and\ distance(obj_{lidar}, obj_{camera}) < distance$\_$limit\\
    and\ absolute(obj_{lidar}.width\ -\ obj_{camera}.width) < width$\_$limit \\ 
    and\ absolute(obj_{lidar}.height\ -\ obj_{camera}.height) < height$\_$limit$}
    {
    $obj_{lidar}.matched = true$\\
    $obj_{camera}.matched = true$\\
    }
    }
  
    }
    \If{$removed=True$}{
    \KwRet Valid\\ 
    %$Valid= True$
    }
    
    \caption{$Checking\ for\ empty\ list\ ,\ \\
    timeouts\ and\ Matching\ between\ \\
    the\ Object\ lists\ CAI\ and\ LAI$}\label{algo_function_monitor_main}
    \end{algorithm}
    \DecMargin{1em}

==> old-texts/backup-evaluation.tex <==
% ------ Implementation Details (original text)
%\subsubsection{Middleware Software Platform}
%To evaluate the software concept of the function monitor, ROS2, the Robot Operating System 2 is utilized. This sophisticated framework enables streamlined publish-subscribe communication, allowing ROS2 nodes to efficiently exchange data in a distributed environment. 

%As detailed in the preceding section, the AI perception validator relies on input from three nodes: safe zone, AI-based camera perception, and AI-based Lidar perception. While the safe zone node is previously established and tested within the function monitor \cite{Felix.2022}, two separate ROS2 nodes AI-based camera perception and AI-based Lidar perception are developed in the environment and self-perception software component. These nodes utilize calibrated sensor data from the Intel RealSense depth camera, employing it in AI-based camera perception to generate a camera AI object list. Similarly, the calibrated sensor data from the Intel RealSense Lidar camera is utilized in AI-based Lidar perception to generate a LiDAR camera AI object list which simulates the LiDAR AI object list. Both perception nodes employ YOLO Nano 2D object detectors \cite{wong2019yolo}, which provide 2D bounding boxes with object class names and confidence scores but lack in providing distance information.

%Given that both perception ROS2 nodes receive point cloud inputs from distinct hardware sensors, the distance of the object is computed using this data. With depth, class names, confidence scores, and bounding box dimensions available, the inputs for the AI Perception validator are complete. Beyond serving the AI Perception validator, these inputs are also subscribed in the Remote Command Control Center for visualizing bounding boxes with class names, confidence, and depth overlaid on the image.

%The AI perception algorithm, residing in a distinct ROS2 node, initially utilizes the safe zone to filter objects within the region of interest and around the vehicle—objects to be considered further in the AI Perception validator algorithm. The output interface of the node is a boolean, indicating whether the camera and Lidar AI object lists are consistent or inconsistent.

%Furthermore, this output is subscribed by a separate node that visualizes the output as a status indicator, displayed in a red box in Figure \ref{fig:person_inside_sz}, within the remote command control centre. A red status indicator signifies inconsistency in the object lists, while a green indicator signals consistency in the AI perception systems.

% --- Scenarios and Hypotheses (original text)
%\textbf{Scenario 1 (H1):} The proposed algorithm accurately identifies consistency when both CAI and LAI object lists detect no objects within ROI. To validate this hypothesis, a wooden human dummy is strategically placed in front of the vehicle, detected by the LAI object list but not by the CAI object list (as illustrated in image 4). The AI perception validator outputs ``consistent'' since the objects are outside the ROI, and the processed object lists are empty. The results of both CAI and LAI object lists, along with the AI perception validator, can be visualized in Figure \ref{fig:person_outside_sz}. The AI perception validation state triggers a green status, indicating ``consistent object lists''.

%\textbf{Scenario 2 (H2):}
%The proposed algorithm correctly identifies consistency when all attributes of all objects match in both CAI and LAI object lists. A traffic light is positioned in front of the vehicle under the ROI, detected by both CAI and LAI object lists (as illustrated in image \ref{fig:traffic_light}). The AI perception validator outputs ``consistent'' since the objects are inside the ROI, and were detected by both sensors. The results of both CAI and LAI object lists, along with the AI perception validator, can be visualized in Figure \ref{fig:traffic_light}. The AI perception validation state triggers a green status, indicating ``consistent object lists''.

%\textbf{Scenario 3 (H3):}
%The proposed algorithm accurately identifies inconsistency when there is at least one inconsistent object in either the CAI or LAI object lists. To validate this hypothesis, a wooden human dummy is placed again in front of the vehicle, but this time in ROI, which is detected by the LAI but not by CAI (as illustrated in image \ref{fig:person_inside_sz}). The results of both CAI and LAI object lists, along with the AI perception validator, can be visualized in Figure \ref{fig:person_inside_sz}. The AI perception validation state triggers a red status, indicating ``inconsistent object lists'' since the objects are within the ROI but not aligned with each other.

% --- Older text version for the scenario-based evaluation
\begin{comment}
\subsection{Scenario-based Qualitative Evaluation}
\label{subsec:evaluation-scenarios}
%\todo T \textbf{TODO}: Text describing the scenarios taken into consideration during the evaluation.
This section begins by presenting the overarching scenario to evaluate the function monitor. Subsequently, it delves into the specific scenario under examination in this work, offering a focused perspective. Lastly, the hypothesis formulated to evaluate the identified scenario is discussed, outlining the key criteria for assessment.

\subsubsection{Overall Scenario}
In the overall scenario, the function monitor undergoes multiple variations. It starts with both the ego vehicle and an object in static positions, gradually introducing complexity by incorporating multiple static objects. The next phase involves maintaining the ego vehicle in a static position while introducing movement to one object, followed by the inclusion of additional moving objects to further amplify complexity.

The assessment then advances to a dynamic ego vehicle scenario, evaluating its performance as the ego vehicle moves while one object remains static. Additional complexity is introduced by incorporating more static objects while the ego vehicle is in motion. The evaluation culminates in a dynamic and intricate scenario where both the ego vehicle and a single object are in motion, subsequently escalating the complexity with multiple dynamic objects moving around within the safe zone.

This work represents the initial phase of the function monitor's evolution, initiating the evaluation with fundamental scenarios. In these foundational tests, the assessment focuses on one object at a time. Initially, both the ego vehicle and the objects are in static positions. Subsequently, the objects are set in motion while the ego vehicle remains static, and vice versa. This variation is designed to assess the fundamental functionalities of the function monitor.

\subsubsection{Focused Scenario}

The Ego vehicle approaches a pickup location to pick up a passenger. Initially, the passenger is standing far from the vehicle, and one of the perception systems detects the passenger as a person. However, as the passenger starts moving closer to the vehicle, one of the perception systems loses track, failing to recognize the passenger. This inconsistency triggers an alert on the remote command and control centre.

The remote operator, alerted to the inconsistency in the AI perception validation state, attentively reviews all sensor data. Simultaneously, the passenger boards the car, and the inconsistency in the AI perception becomes consistent once again. The remote operator, without intervening, observes the sensor data.

The Ego vehicle resumes its journey, encountering a traffic light along the way. Despite the proximity of the traffic light to the vehicle, both perception systems successfully detect it. The vehicle continues driving, reaches its destination, drops off the passenger, and patiently awaits the next mission.

\subsubsection{Hypothesis}

The hypothesis outlined in the given scenario posits that the function monitor is expected to consistently output a "Consistent" status under specific conditions. Firstly, if there is an object detected in either the Camera or Lidar AI object lists, and that object is located outside the safe zone, the function monitor should declare a "Consistent" status. Conversely, if an object is within the safe zone and detected in any one of the object lists, the function monitor is expected to trigger an "Inconsistent" status.

Moreover, the hypothesis states that if the object is identified within the safe zone and is present in both object lists, with the differences in the object properties falling below a defined threshold, the function monitor should declare a "Consistent" status. These conditions serve as the criteria for the expected behaviour and performance of the function monitor in the given scenarios.


To validate the above-stated hypothesis, a wooden person is employed as the test object. Initially, the wooden person is positioned outside the safe zone, and subsequently, it is relocated inside the safe zone, as illustrated in Figure \ref{fig:model_car}. The ego vehicle is then manually manoeuvred to different locations, including where the traffic light is positioned, evaluating the function monitor's performance as the vehicle is in a dynamic state.

As detailed in the previous publication, the safe zone is a combination of the clear and focus zones \cite{Felix.2022}. The parameters for the clear zone are set as follows: Inner: 0.025 m, Outer: 0.025 m, Far: 0.06 m, Near: 0.00 m. In the focus zone, the specified parameters are: Inner: 0.55 m, Outer: 0.55 m, Far: 1.2 m, Near: 0.22 m.

For the comparison of Lidar and camera object lists, specific thresholds are established. The limit timeout is set at 2 seconds or 2000 milliseconds, determining the timeframe for the removal of objects in both the Lidar and the camera local object list. There is no specified threshold for the Class ID or Class name since the detected object should have the same class name. The Euclidean distance is constrained to 0.10 meters, guiding the comparison of Lidar object coordinates with camera object coordinates.

Furthermore, the limit timestamp is defined as 1 second or 1000 milliseconds for comparing Lidar and camera objects. The height of the Lidar object bounding box is restricted to 0.5 meters in comparison to the height of the camera object bounding box. Similarly, the limit width is set at 0.5 meters for comparing the width of Lidar and camera object bounding boxes. These parameters and thresholds contribute to the precise evaluation of the safe zone and the comparison of Lidar and camera object lists in the function monitor.
\end{comment}

% --- Overarching user story from which the scenarios are derived
% --- Nicely formulated text, but due to page limit constraints, this text has not been included in the paper.
%
%In this section, the results are discussed. The ego vehicle reaches a pickup location and waits for the passenger. A wooden person which represents a passenger is positioned 2 meters away from the ego vehicle which is outside the safe zone, as illustrated in the bird's eye view in Figure \ref{fig:model_car}, only one perception system, the Lidar camera-based system, can detect it. The anticipated outcome for the function monitor is consistency, as the object is located outside the safe zone, and only objects within the safe zone are considered by the function monitor. In Figure \ref{fig:person_outside_sz}, the AI perception validation state triggers a green status, indicating consistent object lists.

%When the passenger or the wooden person approaches the ego vehicle and enters the safe zone, and only the Lidar camera-based perception system detects as a person, the expected outcome for the function monitor is inconsistent. Indeed, the AI perception validation state triggers a red status, as shown in Figure \ref{fig:person_inside_sz}, correctly indicating inconsistent object lists in the remote command and control centre. This demonstrates when an object is within the safe zone, and only one perception system detects it, the function monitor responds appropriately.

%The passenger then enters the ego vehicle and the ego vehicle is manoeuvring near the traffic light, both perception systems (depth camera and Lidar camera-based) detect the traffic light as an object. All parameters of the object align with or fall below the specified threshold, and the AI Perception validation state triggers consistent object lists, as shown in the red box in Figure \ref{fig:traffic_light}. This result demonstrates that the function monitor avoids false positives. The ego vehicle then further reaches the destination and waits for the next mission.

%The observed results align with the expectations derived from the hypothesis and the defined scenarios, affirming that the function monitor is operating as intended.

% --- Good text describing the model vehicle and its sensors.
% --- The description of the LiDAR camera and stereo vision camera is very well written and in more detail than in the paper.
% --- Due to page limit constraints, an abridged version of this text has been used in the dexcription of the hardware platform and test track.

%The selected vehicle for evaluating the function monitor concept is a 1:8 scale model vehicle \cite{Mesow_2017}, developed by the company Digitalwerk \cite{Welcomet61:online}. This model vehicle is equipped with a range of sensors, including a mono camera, LiDAR, wheel speed sensor, ultrasonic sensor, GPS, and IMU. Despite the presence of multiple sensors on the model vehicle, the environmental perception is particularly enhanced by the installation of specific sensors. Notably, the Intel RealSense LiDAR camera (L515) and depth camera (D435f) are mounted on the model vehicle, as illustrated in Figure \ref{fig:model_car}.

%The Intel RealSense LiDAR camera (L515) employs LiDAR technology for depth calculation, primarily designed for indoor use. Its specifications include a minimum depth of 0.25 meters up to 9 meters, a depth output resolution of up to $1024 \times 768$, a depth frame rate of 30 fps, and a depth field of view of $70^{\circ} \times 55^{\circ} (\pm 3^{\circ})$ \cite{LiDARCam3:online}.

%On the other hand, the Intel RealSense Depth camera (D435f) utilizes stereoscopic technology for depth calculation, suitable for both indoor and outdoor environments. It features a minimum depth of 0.3 meters up to 3 meters, a depth output resolution of up to $1280 \times 720$, a depth frame rate of up to 90 fps, and a depth field of view of $87^{\circ} \times 58^{\circ}$ \cite{DepthCam5:online}.

%Despite variations in their depth specifications, both cameras share identical RGB specifications, with a frame resolution of $1920 \times 1080$, a standard frame rate of 30 fps, and employ rolling shutter sensor technology with a 2MP RGB sensor resolution. Additionally, both cameras are seamlessly connected via USB-C 3.1. Despite these similarities, their RGB sensor field of view varies, with the Intel RealSense Depth camera having a FOV of $69^{\circ} \times 42^{\circ}$ and the Intel RealSense LiDAR camera featuring a FOV of $70^{\circ} \times 43^{\circ} (\pm 3^{\circ})$ \cite{DepthCam5:online, LiDARCam3:online}.

%All sensors on the model car, including the Intel RealSense cameras, are meticulously calibrated on the rear or back axle of the vehicle to ensure optimal functionality.

==> old-texts/backup-introduction.tex <==
%Text from the SafeWahr Proposal:

%In recent years, a certain structuring of the functional architecture for autonomous vehicles has been established at a high level of abstraction: This includes (1) perception, (2) action planning and (3) motion control [1][2][3]. The perception of the environment (synonym: perception)1 is of particular criticality, as demonstrated not least by the series of accidents in connection with (partially) automated driving functions, e.g. in conjunction with Tesla's Autopilot. In the first accident in 2016, the Tesla Autopilot, which had already driven more than 200 million kilometers by then, failed to detect a trailer crossing a semitrailer truck and collided with it [4]. In response, Tesla questioned the camera system as the leading system for perception at the end of 2016 and announced Shadow Mode2 to prove the safety of Autopilot [5]. A principle of continuous monitoring of autonomous driving functions for development, validation and series operation that fundamentally extends the shadow mode under the two questions (a) does the autonomous driving function work correctly (qualitative oracle) and (b) is the autonomous driving function in a known environment (quantitative oracle), was successfully developed by the applicants as early as mid-2014 using the example of action planning of the aforementioned highway pilot and was demonstrated and published in 2016 [6][7][8].

%However, there is a lack of comprehensive and validated research findings for perception and therefore also for the overall system. Perception is a particular challenge here, as will be shown below.

%A typical procedure for the development of AI-based perception as an essential component of autonomous driving functions is shown in Figure 1. Taking into account the applicable standards, such as ISO 26262 (Functional Safety) and ISO 21448 (Safety of Intended Function, SOTIF) [9][10], a structured process model, such as the V-model, is applied. The starting point for development are (usually incomplete) artifacts: system requirements, AI training data and structured test cases derived from other artifacts, e.g. in the form of OpenSCENARIO, OpenDRIVE and OpenCRG [11][12][13] 
%3.
%Verification and validation take place in parallel, in accordance with the relevant standards and processes, e.g. ISO 26262 and 21448. Development and validation take place iteratively and in stages using verification and validation techniques, as shown in Figure 1. This includes software tests, various stages of software-based simulation, tests on proving grounds, fleet tests and series vehicles with shadow mode. In addition, on-board diagnostics and rudimentary remote monitoring functions are occasionally used in series production.

%This type of development, validation and series operation of autonomous vehicles involves a number of open questions, especially for AI-based perception systems. Further research into methods for continuous monitoring of perception systems for safe release and series operation is required here:

%(1.) For perception, AI-based approaches have prevailed over classical approaches [14][15][16]. AI-based approaches are used both in image processing and in the signal processing of other raw sensor data (e.g. radar). Common standards and approaches for validation, such as ISO 26262 and 21448, are based on the existence of complete requirement specifications. A complete specification of functionality does not usually exist for AI-based perception systems. Instead, extensive AI training data is used. For example, image data with pedestrians is required to train an AI-based pedestrian detection system. Therefore, a new argument is needed that an AI-based perception component is functionally correct and safe. Accepted procedures for such safety proofs do not yet exist. Continuous correctness monitoring during series production can provide such an argument.

%(2.) The closer the "system under test" is to the sensors and the higher the SAE level, the greater the amount of data that needs to be processed in the shortest possible time: At Waymo, over 426 gigabytes (GB) of sensor data are generated per vehicle and kilometer at an average speed of 24 km/h [17]. AVL's Rooftop Box, which is also used by SafeWahr as a prototyping platform, generates 33.3 GB of sensor data per vehicle and kilometer [18]. At the same time, Wachenfeld and Winner postulate a release effort of approx. 6.62 billion kilometers for functions such as the highway pilot [19]5. This means that an astronomical and obviously unattainable 1.53 billion terabytes of data would be required for an absolutely secure release of AI-based perception, as Figure 2 shows. Regardless of whether one fully agrees with this reasoning or not, it is obvious that not all relevant situations can be tested in advance. It remains unclear whether new critical situations are still to be expected in series operation or whether a sufficiently high level of coverage has already been achieved beforehand. Continuous real-time monitoring during validation and series operation enables the vehicle to recognize such situations in good time and react accordingly.

%(3.) Automated vehicles must make reliable decisions under real-time conditions. The decision-making process uses AI-based algorithms. The values of numerous sensors serve as input variables. A (situational) interpretation of the sensor signals is necessary for perception. For example, the AI-based perception must decide whether the detected object is a pedestrian or an advertising pillar with the image of a person. This is essential for further processing, as there is a certain probability that a pedestrian will use the adjacent crosswalk, but not the advertising pillar. From a safety point of view, a second independent calculation path with independent sensors is desirable. Despite redundant sensors, the system needs an additional criterion to decide which path works correctly and correctly represents the real environment. This problem falls into the error class of Byzantine errors, because the system has to make a judgment without knowledge of the environment. Here too, continuous real-time monitoring can provide the system with information on which interpretation is correct and thus guarantee the fail-operational mode.

%Core question of the project: How can continuous real-time monitoring for the safe release and reliable series operation (through self-diagnosis and fail-operational mode) of autonomous vehicles be realized with an AI-based perception system? The monitors are structured and systematically derived from the artifacts of the machine learning process and the requirements specification.
%The following three aspects are continuously monitored by monitors in real time:
%a. Situation monitor: Is the current situation already known and validated during development and validation?
%b. Validity Monitor: How certain is the AI-based environment perception system with regard to its calculated result?
%c. Function Monitor: Is the calculated result within the specified safety properties of the target function?
%At the heart of SafeWahr is a further developed concept of a safety architecture for secure release and reliable series operation. The conceptual basis is the Dependability Cage approach, which has already been tested with the Highway Pilot [20][21]. The artifacts of machine learning and the requirements specification of perception are used to derive its monitors as efficiently and effectively as possible.

%As Figure 3 shows, the core of the advanced safeguarding system is a basic architecture of monitor systems at different levels. These monitors are an indicator of whether the perception is working correctly (qualitative oracle triggers if an indicator comes from the function or validity monitor) and whether the perception has already been sufficiently trained with regard to the current situation (quantitative oracle triggers if an indicator comes from the situation or validity monitor). For series operation, the Dependability Cage thus provides additional on-board monitoring of the target function. The number of kilometers driven in the fleet in relation to the number of faults detected by the monitor (oracle strikes) can be used to determine a measure of the completeness of the protection and thus the safe release. As soon as one of these oracles strikes during series operation, the Perception is no longer in a safe operating state. The autonomous driving system reacts accordingly, in the sense of a fail-operational system, e.g. by selecting (voter) the remaining correct calculation path. This can result in the vehicle handing control back to the driver in an orderly fashion.

%In addition, the resulting operating data (raw sensor data, the calculated result, system status, etc.) is stored, in analogy to a black box or the fault memory of control units, for subsequent more detailed analysis. The situations and operating states identified in this way can then be used later for continuous further development and improvement of the system.

%Hypotheses guiding the research
%Basic hypothesis: Autonomous vehicles cannot be fully validated in advance, as the number of conceivable situations is too high. It is therefore necessary to establish continuous monitoring in order to derive a proof of release and realize self-diagnosis for the series. Partial hypotheses are:
%1. situation monitors can be effectively derived from training data using machine learning to recognize new driving situations in real time.
%2. validity monitors can be effectively derived with the development of AI-based parts to detect unsafe behavior of the developed parts in real time.
%3. function monitors can be systematically derived from requirements via safety properties to monitor the functional safety of the target function in real time.
%4. a fail-operational mode can be realized with the help of the monitors
%5. a methodology for assessing the relevance of the safeguarding runs can be developed to support proof of release.
